Non-linear Redshift-Space Power Spectra

Distances in cosmology are usually inferred from observed redshifts - an estimate that is dependent on the local peculiar motion - giving a distorted view of the three dimensional structure and affecting basic observables such as the correlation function and power spectrum. We calculate the full non-linear redshift-space power spectrum for Gaussian fields, giving results for both the standard flat sky approximation and the directly-observable angular correlation function and angular power spectrum. Coupling between large and small scale modes boosts the power on small scales when the perturbations are small. On larger scales power is slightly suppressed by the velocities perturbations on smaller scales. The analysis is general, but we comment specifically on the implications for future high-redshift observations, and show that the non-linear spectrum has significantly more complicated angular structure than in linear theory. We comment on the implications for using the angular structure to separate cosmological and astrophysical components of 21 cm observations.

==> spt.tex <==

\section{Lagrange Reversion}
Start from Newtonian approximation (drop $\tau_c$) and follow
Richard's notation $\phi = \vv \cdot \vnhat/\clh$ where $\clh$ is
taken to be constant (check scale of validity)
\begin{equation}
\label{eq:dzimpl}
\delta(z) = \left.\frac{\Delta-\phi'}{1+\phi'}\right|_{\chi_z},
\end{equation}
where $\chi_z = \chi - \phi(\chi_z)$ (assume unique solutions
etc). Although we don't need it, the perturbative solution to this
implicit equation for $\chi_z$ is
\begin{equation}
\chi_z = \chi + \left.\sum_{n=0}^\infty \frac{\partial^n}{\partial\chi^n}\left[\frac{(-\phi)^{n+1}}{(n+1)!}\right]\right|_{\chi}.
\end{equation}
This is easily verified for the lowest terms, and follows more
generally from the Lagrange Reversion Theorem\footnote{See
  e.g. \url{http://en.wikipedia.org/wiki/Lagrange_reversion_theorem}}. This
states that if $v$ solves the implicit equation $v=x+yf(v)$ then
\begin{equation}
g(v)=g(x)+\sum_{k=1}^\infty\frac{y^k}{k!} \frac{\partial^{k-1}}{\partial x^{k-1}}\left(f(x)^kg'(x)\right),
\end{equation}
and the result follows from setting $g(x)=x$, $y=1$. We can also apply
the theorem directly to $\delta(z)$ to obtain
\begin{equation}
\delta(z) = \left.\frac{\Delta-\phi'}{1+\phi'}\right|_\chi+  \left.\sum_{k=1}^\infty\frac{1}{k!}\frac{\partial^{k-1}}{\partial \chi^{k-1}} \left[ (-\phi)^k \frac{\partial}{\partial\chi}\left( \frac{\Delta-\phi'}{1+\phi'}\right)\right]\right|_{\chi}.
\end{equation}
Expanding $(1+\phi')^{-1} = \sum_m (-\phi')^m$ and grouping terms of
order $n+1$ this miraculously simplifies to
\begin{equation}
\delta(z) = \left.\sum_{n=0}^\infty \frac{(-1)^n}{n!}\frac{\partial^n}{\partial\chi^n}\left[ (\Delta-\phi')\phi^{n}\right]\right|_{\chi}.
\end{equation}
This should allow us to write a relatively simple non-perturbative
result for the redshift-space power spectrum in terms of $P_z$ (the
1st order redshift-space spectrum), the power spectrum of powers of
the velocity, and the cross-correlation.  The series can also be
written with un-grouped terms as
\begin{equation}
1+\delta(z) = \left.\sum_{n=0}^\infty \frac{(-1)^n}{n!}\frac{\partial^n}{\partial\chi^n}\left[ (1+\Delta)\phi^{n}\right]\right|_{\chi} .
\end{equation}
\section{Power Spectrum}


To calculate the power spectrum we must take the Fourier transform of
the expectation of $\delta(\vx_1)\,\delta(\vx_2)$. The transform of
the pair is:
\begin{multline}
\delta(\vk)\,\delta(\vq)  = \sum_{n,m} \frac{i^{n+m}}{n!\, m!} \left(\vnhat \cdot \vk\right)^n \left(\vnhat \cdot \vq\right)^m (2 \pi)^3 \int \dkp[0] \dotsm \dkp[n] \dqp[0] \dotsm \dqp[m] \\ 
 \shoveright{\mbox{} \times  \left[\Delta(\vk_0) + i \vnhat \cdot \vk_0 \,\phi(\vk_0)\right]\, \left[\Delta(\vq_0) + i \vnhat \cdot \vq_0 \,\phi(\vq_0)\right]\, \phi(\vk_1) \dotsm \phi(\vk_n)\, \phi(\vq_1) \dotsm \phi(\vq_m)} \\[4pt]
 \mbox{} \times \delta(\vk_0 \dotsb + \vk_n - \vk)\, \delta(\vq_0 \dotsb + \vq_m - \vq)
\end{multline}
Writing $\alpha(\vk) = \Delta(\vk) + i\, \vnhat \cdot \vk
\:\phi(\vk)$, and $\vnhat \cdot \vk = \kpar$ for brevity we can
evaluate the expectation. All combinations where $n + m$ is odd
average to zero, and we are left with only the even terms:
\begin{multline}
\bigl\langle\delta(\vk)\,\delta(\vq)\bigr\rangle  = \sum_{n,m} \epsilon_{n+m} \frac{(-1)^{(n+m)/2}}{n!\, m!} \kpar^n \qpar^m (2 \pi)^3 \int \dkp[0] \dotsm \dkp[n] \dqp[0] \dotsm \dqp[m] \\ 
\mbox{} \times  \Bigl\langle\alpha(\vk_0) \, \alpha(\vq_0) \, \phi(\vk_1) \dotsm \phi(\vk_n)\, \phi(\vq_1) \dotsm \phi(\vq_m)\Bigr\rangle\: \delta(\vk_0 \dotsb + \vk_n - \vk)\, \delta(\vq_0 \dotsb + \vq_m - \vq)
\end{multline}
where we have defined $\epsilon_n$ to differentiate between odd and
even arguments:
\begin{equation}
\epsilon_n = \begin{cases} 1 & \text{$n$ even} \\
  0 & \text{$n$ odd}
\end{cases}
\end{equation}

Superposing the two delta functions we can replace $\delta(\vq_0
\dotsb + \vq_m - \vq)$ with $\delta(\vk_0 \dotsb + \vk_n + \vq_0
\dotsb + \vq_m - \vk - \vq)$. Using Wicks theorem to evaluate the
expectation value will generate delta functions containing all pairs
of $\vk_i$, $\vq_i$, this allows us to simplify this delta function to
$\delta(\vk + \vq)$. Give this, we can extract the power spectrum
$P(\vk)$ defined by $\bigl\langle\delta(\vk)\,\delta(\vq)\bigr\rangle
= P(\vk) \delta(\vk + \vq)$ yielding:
\begin{multline}
\label{eq:ps}
P(\vk)  = \sum_{n,m} \epsilon_{n+m} \frac{(-1)^{(n-m)/2}}{n!\, m!} (2 \pi)^3 \kpar^{n+m} \int \dkp[0] \dotsm \dkp[n] \dqp[0] \dotsm \dqp[m] \\ 
\mbox{} \times  \Bigl\langle\alpha(\vk_0) \, \alpha(\vq_0) \, \phi(\vk_1) \dotsm \phi(\vk_n)\, \phi(\vq_1) \dotsm \phi(\vq_m)\Bigr\rangle\: \delta(\vk_0 \dotsb + \vk_n - \vk)
\end{multline}
We would like to be able to express the power spectrum above in terms
of the spectra $P_{\Delta\Delta}$, $P_{\Delta\phi}$ and $P_{\phi\phi}$
defined by:
\begin{align}
\bigl\langle\Delta(\vk)\,\Delta(\vq)\bigr\rangle & = P_{\Delta\Delta}(\vk)\, \delta(\vk + \vq) \\
\bigl\langle\Delta(\vk)\,\phi(\vq)\bigr\rangle & = P_{\Delta\phi}(\vk)\, \delta(\vk + \vq) \\
\bigl\langle\phi(\vk)\,\phi(\vq)\bigr\rangle & = P_{\phi\phi}(\vk)\, \delta(\vk + \vq)
\end{align}
The peculiar velocity field is related to the underlying matter
perturbation via
\begin{equation}
\label{eq:vel}
\vv(\vk) = i \frac{\vk}{k^2} f \mathcal{H} \delta
\end{equation}
where $f$ is the log-derivative of the linear growth factor $f =
d\ln{D(a)}/d\ln{a}$.  From this we can see that $P_{\phi\phi}(\vk) =
\kpar^2 / k^4 P_{\delta\delta}(k)$ is anisotropic but symmetric;
whilst for a statistically isotropic $\Delta$ we find
$P_{\Delta\phi}(\vk) = i \kpar / k^2 P_{\Delta\delta}(\vk)$ is
antisymmetric in $\vk$. Hence
$$\int \dkp P_{\Delta\phi}(\vk)\, S(\vk) = 0$$
where $S(\vk)$ is any symmetric function of $\vk$. This allows us to
write the power spectra $P_{\alpha\alpha}$ and $P_{\alpha\phi}$
(defined in the obvious manner):
\begin{align}
P_{\alpha\alpha}(\vk) & = P_{\Delta\Delta}(\vk) -2 i \kpar P_{\Delta\phi}(\vk) + \kpar^2 P_{\phi\phi}(\vk) \\
P_{\alpha\phi}(\vk) & = P_{\Delta\phi}(\vk) + i \kpar P_{\phi\phi}(\vk)
\end{align}
where $P_{\alpha\alpha}$ is the redshift-space power spectrum at first
order. Further we find that $P_{\alpha\phi}$ is antisymmetric, this
will be useful later on.

The expectation in \eqref{eq:ps} can be split up into terms of
distinct types with the $\alpha$'s being contracted differently. Given
that the expectation is evaluated within the integral, we will
implicitly swap around within the sets of dummy variables $\vk_i$ and
$\vq_i$.
\begin{align}
\Bigl\langle\alpha(\vk_0) \, \alpha(\vq_0) \, \phi(\vk_1) \dotsm \phi(\vk_n)\, \phi(\vq_1) \dotsm \phi(\vq_m)\Bigr\rangle = & \Bigl\langle \alpha(\vk_0) \alpha(\vq_0) \Bigr\rangle\, \Bigl\langle \phi(\vk_1) \dotsm \phi(\vk_n)\Bigr\rangle\, \Bigl\langle \phi(\vq_1) \dotsm \phi(\vq_m)\Bigr\rangle \notag \\
 \mbox{} + n m\, & \Bigl\langle \alpha(\vk_0) \alpha(\vq_0) \Bigr\rangle \, \Bigl\langle \phi(\vk_1) \phi(\vq_1) \Bigr\rangle \, \Bigl\langle \phi(\vk_2) \dotsm \phi(\vk_n)\, \phi(\vq_2) \dotsm \phi(\vq_m)\Bigr\rangle \notag \\
 \mbox{} + n m\, & \Bigl\langle \alpha(\vk_0) \phi(\vk_1) \Bigr\rangle \, \Bigl\langle \alpha(\vq_0) \phi(\vq_1) \Bigr\rangle \, \Bigl\langle \phi(\vk_2) \dotsm \phi(\vk_n)\, \phi(\vq_2) \dotsm \phi(\vq_m)\Bigr\rangle \\
 \mbox{} + n (n -1 )\, & \Bigl\langle \alpha(\vk_0) \phi(\vk_1) \Bigr\rangle \, \Bigl\langle \alpha(\vq_0) \phi(\vk_2) \Bigr\rangle \, \Bigl\langle \phi(\vk_3) \dotsm \phi(\vk_n)\, \phi(\vq_1) \dotsm \phi(\vq_m)\Bigr\rangle \notag \\
 \mbox{} + n m\, & \Bigl\langle \alpha(\vk_0) \phi(\vq_0) \Bigr\rangle \, \Bigl\langle \alpha(\vq_1) \phi(\vk_1) \Bigr\rangle \, \Bigl\langle \phi(\vk_2) \dotsm \phi(\vk_n)\, \phi(\vq_2) \dotsm \phi(\vq_m)\Bigr\rangle \notag \\
 \mbox{} + m (m - 1)\, & \Bigl\langle \alpha(\vk_0) \phi(\vq_1) \Bigr\rangle \, \Bigl\langle \alpha(\vq_0) \phi(\vq_2) \Bigr\rangle \, \Bigl\langle \phi(\vk_2) \dotsm \phi(\vk_n)\, \phi(\vq_3) \dotsm \phi(\vq_m)\Bigr\rangle \notag 
\end{align}
Terms of the form $\left\langle \alpha(\vk_i) \phi(\vk_j)
\right\rangle$, or the similar $\vq$ terms will integrate to zero in
the above because of the antisymmetry of $P_{\alpha\phi}$. That leaves
only the first, second and fifth terms of the above. The first term
appears only for even $n$, and it separates out the integrals
entirely, with the permutations giving $n!\, m!$ identical terms. The
second and fifth terms do not decouple the integrals, however they
contain the common expectation over the $\phi$ simplifying
\eqref{eq:ps} to:
\begin{multline}
P(\vk)  = \sum_{n,m} \epsilon^{n+m} \frac{(-1)^{(n-m)/2}}{n!\, m!} \kpar^{n+m} \Biggl[\epsilon_n \frac{n!}{(\frac{n}{2})! 2^{\frac{n}{2}}}\,\frac{m!}{(\frac{m}{2})! 2^{\frac{m}{2}}} R_{\phi\phi}^{\left(n+m\right)/2} P_{\alpha\alpha}(\vk) + \int \dkp[0] \dotsm \dkp[n] \dqp[2] \dotsm \dqp[m] \\ 
\mbox{} \times \Bigl[P_{\alpha\alpha}(\vk_0) P_{\phi\phi}(\vk_1) - P_{\alpha\phi}(\vk_0) P_{\alpha\phi}(\vk_1) \Bigr] \Bigl\langle \phi(\vk_2) \dotsm \phi(\vk_n)\, \phi(\vq_2) \dotsm \phi(\vq_m)\Bigr\rangle\: \delta(\vk_0 \dotsb + \vk_n - \vk)\Biggr]
\end{multline}
where in the above we have defined:
$$
R_{\phi\phi} = \int \frac{d\vk}{(2\pi)^3} P_{\phi\phi}(\vk)
$$

To calculate the above to increasing orders in the power spectra we
must sum over all sets of $n$,$m$ given $n + m$ is constant. Let us do
this explicitly by changing the summations. We relabel with $r$ and
$s$, such that $r = (n + m)/2$ and $s = n$. With this, the
contribution at $r$-th order, $\presup{(r)}P(\vk)$ are:
\begin{multline}
\label{eq:ps_pert}
\presup{(r)}P(\vk)  = (-1)^r \kpar^{2r} \sum_{s \leqslant 2r} \Biggl[\epsilon_s\,\frac{1}{2^r\,(\frac{s}{2})!\,(r - \frac{s}{2})!} R_{\phi\phi}^r P_{\alpha\alpha}(\vk) \\
\mbox{}+ \frac{(-1)^{s}}{s!\, (2r - s)!} \int \frac{d^3\vk_0\, d^3\vk_1}{(2\pi)^3} \Bigl[P_{\alpha\alpha}(\vk_0) P_{\phi\phi}(\vk_1) - P_{\alpha\phi}(\vk_0) P_{\alpha\phi}(\vk_1) \Bigr] F_{r,s}(\vk - \vk_0 - \vk_1)\Biggr] 
\end{multline}
where we have used:
\begin{align}
F_{r,s}(\vk) & = 0 & \text{$r \leqslant 0$ or $s \leqslant 0$ or $s \geqslant 2r$} \notag \\
& = \delta(\vk) & \text{$r = 1$ and $s = 1$} \notag \\
  & = \int \dqp[1] \dotsm \dqp[2(r-1)] \Bigl\langle \phi(\vq_1) \dotsm \phi(\vq_{2(r-1)})\Bigr\rangle \delta(\vq_1 \dotsb + \vq_{s-1} - \vk) & \text{otherwise}
\end{align}
Further simplification can be made by use of the identity
\begin{equation}
\sum_{k = 0}^n \frac{n!}{k!\,(n - k)!} = 2^n
\end{equation}
in the first summation, and then noting that the resultant terms give
the Taylor expansion of an exponential. We have the final result that
the full power spectrum is given by:
\begin{multline}
P(\vk)  = \exp{\left( - \kpar^2 R_{\phi\phi}\right)} P_{\alpha\alpha}(\vk) \\
\mbox{}+ \sum_{r,s \leqslant 2r} \frac{(-1)^{r+s}}{s!\, (2r - s)!} \kpar^{2r} \int \frac{d^3\vk_0\, d^3\vk_1}{(2\pi)^3} \Bigl[P_{\alpha\alpha}(\vk_0) P_{\phi\phi}(\vk_1) - P_{\alpha\phi}(\vk_0) P_{\alpha\phi}(\vk_1) \Bigr] F_{r,s}(\vk - \vk_0 - \vk_1)
\end{multline}


\section{Second Order Power Spectrum}


In order to evaluate the effects the redshift space distortions, in
the absence of a convenient method of evaluating the sum free form, we
would like the perturbative result to second order. Using
\eqref{eq:ps_pert}, we explicity calculate these contributions. The
lowest order term is simply:
\begin{equation}
\presup{(0)}P(\vk) = P_{\alpha\alpha}(\vk)
\end{equation}
The terms at next order are:
\begin{equation}
\presup{(1)}P(\vk) = -\kpar^2 \biggl[ P_{\alpha\alpha}(\vk) R_{\phi\phi} - \int \dkp[0]\dkp[1] \bigl[P_{\alpha\alpha}(\vk_0) P_{\phi\phi}(\vk_1) - P_{\alpha\phi}(\vk_0) P_{\alpha\phi}(\vk_1) \bigr] \delta(\vk_0 + \vk_1 - \vk) \biggr]
\end{equation}
We should check for divergence at large values of $k$ (where the first
and second terms in the above become large). Given that the
contributions in the integral come from a range of $k_0$ much less
than $k$ when it is large we Taylor expand for $k_0 \ll k$. As $k
\rightarrow \infty$ the rapidly divergent terms cancel, as do
$P_{\alpha\phi}$ at zeroth order, and at first order
$P_{\alpha\alpha}$ (both by symmetry). We are left with:
\begin{equation}
\presup{(1)}P(\vk) = \kpar^2 \int \frac{d^3\vq}{(2\pi)^3} \biggl[\frac{1}{2} P_{\phi\phi}(\vq) \left[\del_a \del_b P_{\alpha\alpha}(\vk)\right] q^a q^b + P_{\alpha\phi}(\vq) \left[\del_a P_{\alpha\phi}(\vk)\right] q^a \biggr]
\end{equation}
where the summation convention applies to latin indices. The above
diverges approximately as some constants times the power spectra. To
see this we define a new variable $\veta(\vk) = \vkhat \ln{k}$ and
transform the derivatives with respect to $\vk$. The transformation
matrix is:
\begin{equation}
\frac{\partial\eta^a}{\partial k^b} = \frac{1}{k}\left[\delta^a_b \eta + \mu^a \mu_b (1-\eta)\right] = \frac{1}{k} X^a_b
\end{equation}
where $\mu_a = k_a / k$. Making the transformation gives:
\begin{multline}
\presup{(1)}P(\vk) = \frac{1}{2} \mu^2 P_{\alpha\alpha}(\vk) \int \frac{d^3\vq}{(2\pi)^3} P_{\phi\phi}(\vq) \left[\frac{\partial^2}{\partial \eta^a \partial \eta^b} \ln{P_{\alpha\alpha}(\vk)} + \pdiff{\eta^a} \ln{P_{\alpha\alpha}(\vk)} \pdiff{\eta^b} \ln{P_{\alpha\alpha}(\vk)}\right] X^a_c X^b_d q^c q^d \\
+ \mu^2 \left(k P_{\alpha\phi}(\vk)\right) \int \frac{d^3\vq}{(2\pi)^3} P_{\alpha\phi}(\vq) \left[\pdiff{\eta^a} \ln{\left(k P_{\alpha\phi}(\vk)\right)} + \hat{k}_a\right] X^a_b q^b
\end{multline}
where the terms in square brackets are almost constant with respect to
$k$, and have a slow angular dependence. The two terms yield integrals
over the matter power spectrum with some angular dependence, giving a
logarithmic divergence.

To specialise this to the case of the matter power spectrum where
$\Delta = \delta$, we use \eqref{eq:vel} noting that in the region of
interest we are in matter domination and $f = 1$. The power spectrum
reduces to:
\begin{align}
\presup{(0)}P(\vk) & = P(k) \left[1 + \mu^2\right]^2 \\
\presup{(1)}P(\vk) & = -\mu^2 k^2 P(k) \left(1 + f\mu^2\right)^2 R_{\phi\phi} \notag \\
& \mbox{} + \mu^2 k^2 \int \frac{d\vq}{(2\pi)^3} P(q)P(\left\lvert\vk - \vq\right\rvert) \Biggl[\frac{\qpar^2}{q^4} +\frac{\qpar \left(\kpar - \qpar\right)}{q^2 \left|\vk - \vq\right|^2}
+2 \frac{\kpar \qpar \left(\kpar - \qpar\right)^2}{q^2 \left|\vk - \vq\right|^4} +\frac{\kpar \qpar^2 \left(\kpar - \qpar\right)^3}{q^4 \left|\vk - \vq\right|^4} \Biggr]
\end{align}
Symmetrising the terms with respect to changes $\vq$ and $\vk - \vq$,
combining the first and second terms and writing $\vp = \vk - \vq$:
\begin{align}
\presup{(1)}P(\vk) & = \mu^2 k^2 P(k) \left(1 + f\mu^2\right)^2 R_{\phi\phi} \notag \\
& \mbox{} + \frac{1}{2} \mu^2 k^2 \int \frac{d\vq d\vp}{(2\pi)^3} P(q)P(p)\Biggl[\frac{\qpar^2}{q^4} + \frac{\ppar^2}{p^4} + 2\frac{\qpar \ppar}{q^2 p^2} + 2\frac{\kpar \qpar \ppar^2}{q^2 p^4} + 2\frac{\kpar \qpar^2 \ppar}{q^4 p^2}+\frac{\kpar \qpar^2 \ppar^3}{q^4 p^4} +\frac{\kpar \qpar^3 \ppar^2}{q^4 p^4}\Biggr] \delta(\vq + \vp - \vk)
\end{align}

\section{Calculating Correlation Functions}


Defining what is effectively the half-cosine transform of
the radial power spectrum:
\begin{equation}
D_n(r) = \frac{1}{2 \pi^2} \int^{\infty}_0\! dk\, \cos{(k r)}\, \bigl[k^{2-n} P(k)\bigr]
\end{equation}
the first two derivatives of $C_n(r)$ are succintly expressed as:
\begin{align}
\frac{d}{dr}C_n(r) &= \frac{1}{r}\Bigl[D_n(r) - C_n(r)\Bigr] & \frac{d^2}{dr^2}C_n(r) & = \frac{2}{r^2}\Bigl[C_n(r) - D_n(r)\Bigr] - C_{n-2}(r)
\end{align}
% \biggl[\frac{2}{\pi}\biggr]^{\frac{1}{2}}

